Linearized Optimal Power Flow for Multiphase Radial Networks with Delta Connections

This paper proposes a linear approximation of the alternating current optimal power flow problem for multiphase distribution networks with voltage-dependent loads connected in both wye and delta configurations. We establish a set of linear equations that exactly describes the relationship between power changes at a bus and the corresponding values from a delta-connected device under specific assumptions necessary for a widely accepted linear model. Numerical studies on IEEE test feeders demonstrate that the proposed linear model provides solutions with reasonable error bounds efficiently, as compared with an exact nonconvex formulation and a convex conic relaxation. Our experiments reveal that modeling delta-connected, voltage-dependent loads as if they are wye-connected can lead to significantly different voltage profiles. We also investigate the limitations of the proposed linear approximation stemming from the underlying assumptions, while emphasizing its robust performance in practical situations.

==> reference.tex <==

@inproceedings{gan2014convex,
  title={Convex relaxations and linear approximation for optimal power flow in multiphase radial networks},
  author={Gan, Lingwen and Low, Steven H},
  booktitle={2014 Power Systems Computation Conference},
  pages={1--9},
  year={2014},
  organization={IEEE}
}

@techreport{schneider2010evaluation,
  title={Evaluation of conservation voltage reduction {(CVR)} on a national level},
  author={Schneider, Kevin P and Fuller, Jason C and Tuffner, Francis K and Singh, Ruchi},
  year={2010},
  institution={Pacific Northwest National Lab.(PNNL), Richland, WA (United States)}
}

@inproceedings{rigoni2020open,
  title={{Open-DSOPF}: An open-source optimal power flow formulation integrated with {OpenDSS}},
  author={Rigoni, Valentin and Keane, Andrew},
  booktitle={2020 IEEE Power \& Energy Society General Meeting (PESGM)},
  pages={1--5},
  year={2020},
  organization={IEEE}
}

@article{fobes2020powermodelsdistribution,
  title={{PowerModelsDistribution. jl: An} open-source framework for exploring distribution power flow formulations},
  author={Fobes, David M and Claeys, Sander and Geth, Frederik and Coffrin, Carleton},
  journal={Electric Power Systems Research},
  volume={189},
  pages={106664},
  year={2020},
  publisher={Elsevier}
}

@article{claeys2021voltage,
  title={Voltage-dependent load models in unbalanced optimal power flow using power cones},
  author={Claeys, Sander and Deconinck, Geert and Geth, Frederik},
  journal={IEEE Transactions on Smart Grid},
  volume={12},
  number={4},
  pages={2890--2902},
  year={2021},
  publisher={IEEE}
}
